Prompt a Robot to Walk with Large Language Models

Large language models (LLMs) pre-trained on vast internet-scale data have showcased remarkable capabilities across diverse domains. Recently, there has been escalating interest in deploying LLMs for robotics, aiming to harness the power of foundation models in real-world settings. However, this approach faces significant challenges, particularly in grounding these models in the physical world and in generating dynamic robot motions. To address these issues, we introduce a novel paradigm in which we use few-shot prompts collected from the physical environment, enabling the LLM to autoregressively generate low-level control commands for robots without task-specific fine-tuning. Experiments across various robots and environments validate that our method can effectively prompt a robot to walk. We thus illustrate how LLMs can proficiently function as low-level feedback controllers for dynamic motion control even in high-dimensional robotic systems. The project website and source code can be found at: https://prompt2walk.github.io/ .

==> sections/introduction.tex <==
\section{INTRODUCTION}
% \subsection{Large Language Models from Control Perspective} 

Large language models (LLMs), pre-trained on internet-scale data \cite{brown2020language, radford2019language, radford2018improving, devlin2018bert, vaswani2017attention} have demonstrated impressive results in various fields, such as natural language processing \cite{ouyang2022training, openai2023gpt}, computer vision \cite{radford2021learning}, and code generation \cite{chen2021evaluating}. LLMs operate by generating information token by token, where each token often corresponds to a word or part of a word. A critical step in this generative process can be mathematically expressed as $\arg\max_{w_{n+1}}P_r(w_{n+1} | w_1, w_2, \ldots, w_n)$, where $P_r(w_{n+1} | w_1, w_2, \ldots, w_n)$ denotes the probability of the next word $w_{n+1}$ given the sequence of preceding words $w_1, w_2, \ldots, w_n$. This process iterates until the model produces a termination token, signifying the end of the generation. To enhance the ability to predict the next token, LLMs undergo training on large datasets, fine-tuning on more specific data for targeted tasks, and prompting, where user-provided inputs $w_1, w_2, \ldots, w_k$ guide the model's output generation. This approach, especially prompting, enables LLMs to perform zero or few-shot learning, adapting to new tasks without direct training by leveraging LLMs' extensive knowledge with few examples as the user's context-specific prompts. Moreover, prompting allows grounding LLMs to enhance their understanding and generation capabilities by linking their outputs to real-world knowledge and context.


%The probability function crucial for generating the next token in LLMs is honed through training, fine-tuning, and prompting. Training teaches the model to predict token probabilities using a large text dataset and advanced learning techniques. Fine-tuning then adjusts the pre-trained model with a smaller, specific dataset to enhance its performance on targeted tasks without losing general language skills. Prompting, without modifying the pre-trained model, uses crafted inputs, which are given $w_1, w_2, \ldots, w_k$ by the user, to guide output generation, exploiting the model's learned patterns for diverse applications efficiently.

Recently, building upon the success of LLMs, there is a surging interest in utilizing LLMs for embodied agents \cite{ahn2022can, vemprala2023chatgpt}, aiming to harness the power of foundation models in the physical world \cite{bommasani2021opportunities}. Towards this goal, significant progress has been made \cite{brohan2022rt, brohan2023rt, driess2023palm}. However, foundation models previously performed low-level control, e.g., target joint positions, which were generally based on training or fine-tuning using significant volumes of robot data.

\begin{figure}
    \centering
    \includegraphics[trim={0.0cm 3.2cm 0.0cm 0.0cm},clip,width=1.0\linewidth]{figs/demo.pdf}
    \caption{\textbf{Prompt a Robot to Walk.} Grounded in a physics-based simulator, LLMs output target joint positions to enable a robot to walk given a text prompt, which consists of a description prompt and an observation and action prompt.}
    \label{fig:cover}
    \vspace{-0.15in}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/method.pdf}
    \caption{\textbf{LLM Policy Overview.} We first collect data from an existing controller to initialize the LLM policy. Then, we design a text prompt including a description prompt and an observation and action prompt. The LLM outputs normalized target joint positions that are then tracked by a PD controller. After each LLM inference loop, the prompt is updated with the historical observations and actions. In our experiment, the LLM is supposed to run at $10$ Hz although the simulation has to be paused to wait for LLM inference, and the PD controller executes at $200$ Hz.}
    \label{fig:method}
    \vspace{-0.15in}
\end{figure*}

Therefore, we raise an intriguing question of whether LLMs can function as low-level controllers, which output the target joint position directly, for achieving dynamic tasks like robots walking through prompting. We explore a new paradigm that leverages few-shot prompts with a large language model, i.e., GPT-4, to output robot control actions directly. To be more specific, here, we utilize LLMs as model predictive control (MPC), diverging from the conventional approach of employing them primarily as planners. We hypothesize that, given prompts collected from the physical environment, LLMs can learn to interact with it in context, even though they are purely trained on text data. Moreover, we do not perform any fine-tuning of the LLM with task-specific robot data. We adopt a few-shot prompt approach, which contains historical observation and actions, and is widely adopted in the natural language field. Furthermore, we consider a dynamic control task of robot walking. 
A visualization of the paradigm is illustrated in Fig.~\ref{fig:cover}. We term this paradigm as prompting a robot to walk. Grounded in a physical environment, LLMs output target joint positions to allow a robot to walk given a designed text prompt, which includes a description prompt and an observation and action prompt. Consequently, the robot is able to interact with the physical world through the generated control actions and get the observations from the environment. In summary, the contributions are as follows:
\begin{itemize}
    \item Our main contribution is a framework for prompting a robot to walk with LLMs, where LLMs act as a feedback policy rather than a planner as is common in recent work.
    \item We propose and systematically analyze a text prompt design that enables LLMs to in-context learn robot walking behaviors.
    \item We extensively validate our framework on different robots, various terrains, and multiple simulators.
\end{itemize}
